Truthful Mechanisms for Combinatorial Allocation of Electric Power in Alternating Current Electric Systems for Smart Grid

Traditional studies of combinatorial auctions often only consider linear constraints. The rise of smart grid presents a new class of auctions, characterized by quadratic constraints. This paper studies the {\em complex-demand knapsack problem}, in which the demands are complex valued and the capacity of supplies is described by the magnitude of total complex-valued demand. This naturally captures the power constraints in alternating current (AC) electric systems. In this paper, we provide a more complete study and generalize the problem to the multi-minded version, beyond the previously known $\frac{1}{2}$-approximation algorithm for only a subclass of the problem. More precisely, we give a truthful PTAS for the case $\phi\in[0,\frac{\pi}{2}-\delta]$, and a truthful FPTAS, which {\it fully} optimizes the objective function but violates the capacity constraint by at most $(1+\epsilon)$, for the case $\phi\in(\frac{\pi}{2},\pi-\delta]$, where $\phi$ is the maximum argument of any complex-valued demand and $\epsilon,\delta>0$ are arbitrarily small constants. We complement these results by showing that, unless P=NP, neither a PTAS for the case $\phi\in(\frac{\pi}{2},\pi-\delta]$ nor any bi-criteria approximation algorithm with polynomial guarantees for the case when $\phi$ is arbitrarily close to $\pi$ (that is, when $\delta$ is arbitrarily close to $0$) can exist.

==> bi-fptas.tex <==
\section{Bi-criteria FPTAS for \textsc{CKP$[0,\pi-\delta]$}} \label{sec:bfptas} 

In the previous section, we have restricted our attention to the setting where all demands lie in the positive quadrant in the complex plane (i.e., \textsc{CKP$[0,\frac{\pi}{2}]$}). In this section, we extend our study to the second quadrant (\textsc{CKP$[0,\pi-\delta]$}) for any $\delta > 0$, that is, we assume ${\rm arg}(d_k) \le \pi-\delta$ for all $k \in \cN$. We note that the next section shows that \textsc{CKP$[0, \pi]$} is inapproximable and 
there is no $(\alpha, 1)$-approximation for \textsc{CKP$[0,\pi - \delta]$}. Therefore, we can at best obtain a bi-criteria approximation, and furthermore the running time should depend on the maximum angle $\phi\triangleq\max_k{\rm arg}(d_k)$.

For convenience, we let $\theta = \max\{\phi - \frac{\pi}{2},0\}$
%, such that ${\rm arg}(d_k) \le \theta + \frac{\pi}{2}$ for all $k \in \cN$
 (see Fig.~\ref{f4} for an illustration).
\begin{figure}[!htb]
	\begin{center}
		\includegraphics{fig/fig4.pdf}
	\end{center}
\caption{All demands lie in the shaded area. We measure $\theta = \phi - \frac{\pi}{2}$ from the imaginary axis.}
	\label{f4}
\end{figure}
 

We present a  $(1,1+\epsilon)$-approximation  for \textsc{CKP$[0,\pi-\delta]$} in Algorithm {\sc CKP-biFPTAS} that is polynomial in both $\frac{1}{\epsilon}$ and $n$ (i.e., FPTAS). We assume that $\tan \theta$ is bounded polynomial $P(n)\ge 1$ in $n$; as we will see in the next section, without this assumption, a bi-criteria FPTAS is unlikely to exist. 

Let $\cN_+\triangleq \{k \in \cN \mid d_k^{\rm R} \ge 0\}$ and $\cN_-\triangleq\{k \in \cN \mid d_k^{\rm R} < 0\}$ be the subsets of users with demands in the first and second quadrants respectively. Consider any  solution $S$ to \textsc{CKP$[0,\pi-\delta]$} and define $S_+ \triangleq \{ k \mid d_k^{\rm R} \ge 0, k \in S \}$ and $S_- \triangleq \{ k \mid   d_k^{\rm R} < 0, k \in S \}$ as the subsets of users with demands having non-negative and negative real components respectively. 

The basic idea of Algorithm {\sc CKP-biFPTAS} is to enumerate the guessed total projections on real and imaginary axes for $S_+^\ast$ and $S_-^\ast$ respectively. 
We can use $\tan \theta$ to upper bound the total projections for any feasible subset $S$ as follows:
\begin{align}
 \sum_{k \in S} d_k^{\rm I} \le C, \quad
 \sum_{k \in S_- } - d_k^{\rm R}   \le  C \tan \theta, \quad 
 \sum_{k \in S_+}  d_k^{\rm R}   &\le C(1+ \tan \theta). \label{eq:ubounds}
\end{align}
We then solve two separate {\sc 2DKP} problems (one for each quadrant) to find subsets of demands that satisfy the individual guessed total projections. But since {\sc 2DKP} is generally NP-hard, we need to round-up the demands to get a problem that can be solved efficiently by dynamic programming. We show that the violation of the optimal solution to the rounded problem w.r.t. to the original problem is small in $\epsilon$. 

Next, we describe the rounding in detail. First, we define\footnote{For a more efficient procedure, we may replace $P(n)$ by $\max\{\tan \theta,1\}$; however, choosing $L$ to depend only on $P(n)$, and thus independent of the demands, will be needed for the truthful mechanism in Sec. \ref{sec:tbp}} $L \triangleq \frac{\epsilon C}{n (P(n)+1)}$, such that the new rounded-up demands $\hat{d_k}$ are defined by:
\begin{equation}
\hat d_k =
\hat d_k^{\rm R} + {\bf i} \hat d_k^{\rm I} \triangleq 
\left\{\begin{array}{ll}
\left\lceil \frac{d_k^{\rm R}}{L} \right\rceil \cdot L + {\bf i} \left\lceil \frac{d_k^{\rm I}}{L} \right\rceil \cdot L, &\text{ if }d^{\rm R}_k\ge 0,\\[3mm]
\left\lfloor \frac{d_k^{\rm R}}{L} \right\rfloor \cdot L + {\bf i} \left\lceil \frac{d_k^{\rm I}}{L} \right\rceil \cdot L, & \text{ otherwise. } 
\end{array}\right.
\label{eq:truc}
\end{equation}
Let $\xi_+$ (and $\xi_-$), $\zeta_+$ (and $\zeta_-$) be respectively the guessed real and imaginary absolute total projections of the rounded demands in $S^\ast_+$ (and $S_-^\ast$).
%\begin{equation}
%\xi_+ \triangleq \{ d_k^{\rm R} \mid  k \in S_+ \}, \  \zeta_+ \triangleq \{ d_k^{\rm I} \mid  k \in S_+ \}, \ \xi_- \triangleq \{ - d_k^{\rm R} \mid  k \in S_- \}, \  \zeta_- \triangleq \{ %d_k^{\rm I} \mid  k \in S_- \}
%\end{equation}
Then the possible values of $\xi_+, \xi_-, \zeta_+$ and $\zeta_-$ are integer mutiples of $L$:
\begin{align}
 \xi_+ \in {\cal A}_+ & \triangleq \left\{0, L, 2L,\ldots,\left\lceil \frac{C (1 + P(n) )}{L} \right\rceil \cdot L\right\},\ 
\xi_- \in {\cal A}_- \triangleq \left\{0,L, 2L,\ldots, \left\lceil \frac{C \cdot P(n) }{L} \right\rceil\cdot L \right\}, \nonumber \\
\zeta_+,\zeta_-  \in {\cal B} & \triangleq \left\{0, L, 2L,\ldots,\left\lceil \frac{C}{L} \right\rceil\cdot L.\right\}
\label{eq:grid}
\end{align}
%Note that a feasible guess of total projections should satisfy constraint Eqn.~\raf{C1} for \textsc{CKP}, and thus:
%\begin{equation}\label{eq:sat}
%(\xi_+ - \xi_-)^2 + (\zeta_+ + \zeta_-)^2 \le (1+2\epsilon)^2C^2;
%\end{equation}
%see Lemma~\ref{lem-trunc} below. 
%Step \ref{alg:tight} forces the corresponding selected demands to be tight; otherwise, constraint Eqn.~\raf{C1} could be violated largely. Now, for each guess, we consider solving two {\sc 2DKP} instances separately. The first one with capacities $\xi_+$, $\zeta_+$ and positive demands $\hat d_k, k \in \cN_+$, and the second with $\xi_-,\zeta_-$ and demands in $\cN_-$. 


The next step is to solve the rounded instance exactly. Assume an arbitrary order on $\cN = \{ 1, ..., n\}$. We use recursion to define a 3D table, with each entry ${U}(k,c_1, c_2)$ as the maximum utility obtained from a subset of users $\{1,2,\dots,k\} \subseteq \cN$ with demands $\{\hat{d_1},\hat{d_2},...,\hat{d_k}\}$ that can fit exactly (i.e., satisfies the capacity constraint as an equation) within capacity $c_1$ on the real axis and $c_2$ on the imaginary axis. 
\iffalse
The cells are defined according to the following rules:
\begin{align}
{U}(1,C_1, C_2) &\triangleq  \left\{ \begin{array}{l l}
u_k & \quad \text{if $\hat{d_k^{\rm R}} = C_1$ and $\hat d_k^{\rm I}  = C_2$}\\
-\infty &\quad \text{otherwise} \end{array}\right.\label{eq:dyn-rule1}\\
{U}(i+1,C_1, C_2) &\triangleq \max  \left\{ \begin{array}{l}
u_{i+1} + {U}(i, C_1 - \hat d_k^{\rm R}, C_2 - \hat d_k^{\rm I}),\\
{U}(i,C_1,C_2)
 \end{array}\right.
 \label{eq:dyn-rule2}
\end{align}
\fi
We denote by {\sc 2DKP-Exact}$[\cdot]$ the algorithm for solving {\sc 2DKP} by dynamic programming.


\begin{algorithm}[!htb]
\caption{{\sc CKP-biFPTAS} $( \{u_k,d_k\}_{k \in \cN}, C,\epsilon) $}\label{CKP-biFPTAS}
\begin{algorithmic}[1]
\Require Users' utilities and demands $\{u_k,d_k\}_{k\in \cN}$; capacity $C$; accuracy parameter $\epsilon$
\Ensure $(1,1+3\epsilon)$-solution $\hat{S}$ to \textsc{CKP$[0,\pi-\delta]$}
\State $\hat{S} \leftarrow \varnothing$.
\ForAll {$d_k$ and $k \in \cN$}
\State Set $\hat d_k \leftarrow \hat d_k^{\rm R} + {\bf i} \hat d_k^{\rm I} $ as defined by \raf{eq:truc}
\EndFor
\ForAll {$\xi_+ \in {\cal A}_+, \xi_- \in {\cal A}_-, \zeta_+, \zeta_- \in {\cal B}$}
\If {$(\xi_+ - \xi_-)^2 + (\zeta_+ + \zeta_-)^2 \le (1+2\epsilon)^2C^2$}\label{cond1}
\State $\qquad F_+ \leftarrow \text{\sc 2DKP-Exact}(\{u_k,\hat d_k/L\}_{k\in\cN_+}, \xi_+/L,\zeta_+/L)$
 \State $\qquad F_- \leftarrow \text{\sc 2DKP-Exact}(\{u_k,-\hat d_k/L\}_{k\in \cN_-}, \xi_-/L,\zeta_-/L)$ 
%\If{$F_+, F_- \neq \varnothing$} \label{alg:tight}
\If{$u(F_+ \cup F_-) > u (\hat{S})$}
\State $\hat{S} \leftarrow  \{F_+ \cup F_-\}$
\EndIf 
%\EndIf 
\EndIf
\EndFor
\State \Return $\hat{S}$
\end{algorithmic}
\end{algorithm}


\begin{algorithm}[!htb]
\caption{{\sc 2DKP-Exact} $( \{u_k,\hat d_k\}_{k \in \cN'}, C_1,C_2) $}
\begin{algorithmic}[1] 
\Require Users' utilities and integer demands $\{u_k,\hat d_k\}_{k\in \cN'}$; integer capacities $C_1,C_2$
\Ensure A utility-maximizing subset of satisfiable users $\subseteq \cN'$ subject to capacity constraints defined by $C_1,C_2$
\State Create a 3D table of size $|\cN'| \times (C_1+1) \times (C_2+1)$, with each entry ${U}(k,c_1, c_2)$ according to: 
\begin{align}
{U}(1,c_1, c_2) &\triangleq  \left\{ \begin{array}{l l}
u_1 & \quad \text{if $\hat d_1^{\rm R} = c_1$ and $\hat d_1^{\rm I}  = c_2$}\\
-\infty &\quad \text{otherwise} \end{array}\right.\label{eq:dyn-rule1}\\
U(k, 0, 0) &\triangleq 0 ~~\text{ and }~~U(k, c_1', c_2') \triangleq -\infty\text{ for all }c_1'<0 \text{ or } c_2'<0\\
{U}(k,c_1, c_2) &\triangleq \max  \left\{ 
u_{k} + {U}(k-1, c_1 - \hat d_k^{\rm R}, c_2 - \hat d_k^{\rm I}),
{U}(k-1,c_1,c_2) \right\}
 \label{eq:dyn-rule2}
\end{align}
\State Create a 3D table of size $|\cN'| \times C_1 \times C_2$, with each each entry ${\cI}(k,c_1, c_2)$ according to: 
\begin{align}
\cI(1,c_1, c_2) &\triangleq \left\{\begin{array}{l l}
\{1 \}& \ \text{if $U(1,c_1,c_2) = u_1$}\\
\varnothing & \ \text{otherwise} 
\end{array}\right.\\
{\cI}(k,c_1, c_2) &\triangleq  \left\{ \begin{array}{ll}
{\cI}(k-1,c_1, c_2) &\  \text{if ${U}(k,c_1, c_2) = {U}(k-1, c_1, c_2)$} \\
{\cI}(k-1,c_1- \hat d_k^{\rm R}, c_2- \hat d_k^{\rm I}) \cup \{ k \} &\  \text{if ${U}(k,c_1, c_2) = u_{k} + {U}(k-1, c_1 - \hat d_k^{\rm R}$}, c_2 - \hat d_k^{\rm I}) \\
\end{array}\right.
 \label{eq:dyn-rule3}
\end{align}
\State \Return $\displaystyle {\cI}(n,C_1,C_2)$.
\end{algorithmic}
\end{algorithm}


\begin{theorem}\label{thm:bptas}
Algorithm {\sc CKP-biFPTAS} is $(1,1+3\epsilon)$-approximation for \textsc{CKP$[0,\pi-\delta]$} and its running time is polynomial in both $n$ and $\frac{1}{\epsilon}$.
\end{theorem}
\begin{proof}
First, the running time is proportional to the number of guesses, upper bounded by $O(\frac{1}{\epsilon^4} n^{4} P^6(n))$. For each guess, {\sc 2DKP-Exact} constructs a table of size at most $O(\frac{1}{\epsilon^2} n^3 P^4(n))$. Since we assumed $P(n)$ is polynomial in $n$, the total running time is polynomial in $n$ and $\frac{1}{\epsilon}$.

To show the approximation ratio of 1, we note {\sc CKP-biFPTAS} enumerates over all possible rounded projections subject to the capacity constraint in {\sc CKP} and that {\sc 2DKP-Exact} returns the exact optimal solution for each rounded problem. In particular, by Lemma \ref{lem-trunc} one of the choices would be rounded projection for the optimum solution $S^\ast$.   
It remains to show that the violation of the returned solution is small in $\epsilon$. This is given in Lemma~\ref{lem-trunc2} below, which shows that the solution $\hat S$ to the rounded problem violates the capacity constraint by only a factor at most $(1+3\epsilon)$. 
\end{proof}

%In fact, $\epsilon$ is inversely proportional to $\theta$. The larger $\theta$ the smaller $\epsilon$ is required for maintaining the precision. This can be observed from Eqn.~\raf{lem1-p2}.

For any set $S\subseteq\cN$, let us write $D_+(S)\triangleq\sum_{k\in S_+}d_k^{\rm R}$, $D_-(S)\triangleq\sum_{k\in S_-}-d_k^{\rm R}$, $D_I(S)\triangleq\sum_{k\in S}d_k^{\rm I}$, $\hat D_+(S)\triangleq\sum_{k\in S_+} \hat d_k^{\rm R}$, $\hat D_-(S)\triangleq\sum_{k\in S_-} -\hat d_k^{\rm R}$, and $\hat D_I(S)\triangleq\sum_{k\in S}\hat d_k^{\rm I}$. Then by \raf{eq:truc} and the fact that $x \le t \lceil \frac{x}{t} \rceil  \le x + t$ for any $x,t$ such that $t>0$, we have 
\begin{eqnarray}\label{eq:bds}
&\max\{\hat D_+(S)-L|S|,0\}\le D_+(S)\le \hat D_+(S),~~~\max\{\hat D_-(S)-L|S|,0\}\le D_-(S)\le \hat D_-(S), \nonumber \\ & \max\{\hat D_I(S)-L|S|,0\}\le D_I(S)\le\hat D_I(S).
\end{eqnarray}

\begin{lemma}
For any optimal solution $S^*$ to \textsc{CKP$[0,\pi-\delta]$}, $L\triangleq \frac{\epsilon C}{nP(n)}$ and $\epsilon> 0$, we have
\begin{equation}
 \left( \sum_{k \in S^*} \hat d_k^{\rm R} \right)^2 +  \left(\sum_{k \in S^*} \hat   d_k^{\rm I} \right)^2  \le C^2 ( 1 + 2\epsilon)^2 .
 \label{eq:lem}
\end{equation}
 \label{lem-trunc}
\end{lemma}
\begin{proof}
%First, we note that any optimal solution $S^*$ satisfies constraint Eqn.~\raf{C1}:
%\begin{equation}
%\left(\sum_{k\in S^*} d_k^{\rm R} \right)^2 + \left( \sum_{k \in S^* } d_k^{\rm I}\right)^2 \le C^2
%\label{eq:C1}
%\end{equation}


Using~\raf{eq:bds},
\begin{align}
\left( \sum_{k \in S^*} \hat d_k^{\rm R} \right)^2 +  \left(\sum_{k \in S^*} \hat d_k^{\rm I} \right)^2 &=\left(\hat D_+(S^*)- \hat D_-(S^*)\right)^2 +  \hat D_I^2(S^*)\nonumber\\
&=\hat D_+^2(S^*)+\hat D_-^2(S^*)-2\hat D_+(S^*)\hat D_-(S^*)+\hat D_I^2(S^*)\nonumber\\ 
&\le (D_+(S^*)+nL)^2+(D_-(S^*)+nL)^2-2D_+(S^*) D_-(S^*)+(D_I(S^*)+nL)^2\nonumber\\
&=(D_+(S^*)-D_-(S^*))^2+D_I^2(S^*)+2nL (D_+(S^*)+D_-(S^*)+D_I(S^*))+3n^2L^2\nonumber\\
&= \left(\sum_{k\in S^*} d_k^{\rm R} \right)^2 + \left(\sum_{k\in S^*} d_k^{\rm I}  \right)^2 +2nL\left(\sum_{k\in S^*}|d_k^{\rm R}|+\sum_{k\in S^*}d_k^{\rm I}\right)+3n^2L^2\nonumber\\
&\le C^2 + 4nL (P(n)+1) C + 3n^2L^2 = C^2 + 4 \epsilon C^2 + 3\epsilon^2 C^2/(1+P(n))^2\nonumber \\ &\le C^2 (1+4\epsilon + \epsilon^2)\le C^2(1+2\epsilon)^2.
\end{align}
\end{proof}

\begin{lemma}\label{lem-trunc2}
Let $\hat S$ be the solution returned by {\sc CKP-biFPTAS}. Then $|\sum_{k\in\hat S}d_k|\le(1+3\epsilon) C$. 
\end{lemma}
\begin{proof}
As in~\raf{lem1-p2},
\begin{align}\label{eq:ee1}
\left( \sum_{k \in \hat S} d_k^{\rm R} \right)^2 +  \left(\sum_{k \in \hat S} d_k^{\rm I} \right)^2 &=\left(D_+(\hat S)- D_-(\hat S)\right)^2 +  D_I^2(\hat S)\nonumber\\
&=D_+^2(\hat S)+D_-^2(\hat S)-2D_+(\hat S)D_-(\hat S)+D_I^2(\hat S).
\end{align} 
If both $\hat D_+(\hat S)$ and $\hat D_-(\hat S)$  are less than $nL$, then the R.H.S. of \raf{eq:ee1} can be bounded by 
\begin{align}\label{eq:ee2}
&\hat D_+^2(\hat S)+\hat D_-^2(\hat S)+\hat D_I^2(\hat S)
\le\hat D_+^2(\hat S)+\hat D_-^2(\hat S)-2\hat D_+(\hat S)\hat D_-(\hat S)+2n^2L^2+\hat D_I^2(\hat S)\nonumber\\
&=(\hat D_+(\hat S)-\hat D_-(\hat S))^2+\hat D_I^2(\hat S)+2n^2L^2.
\end{align}
Otherwise, we bound the R.H.S. of \raf{eq:ee1} by
\begin{align}\label{eq:ee3}
&\hat D_+^2(\hat S)+\hat D_-^2(\hat S)-2(\hat D_+(\hat S)-nL)(\hat D_-(\hat S)-nL)+\hat D_I^2(\hat S)\nonumber\\
&=(\hat D_+(\hat S)-\hat D_-(\hat S))^2+\hat D_I^2(\hat S)+2nL(\hat D_+(\hat S)+\hat D_-(\hat S))-2n^2L^2.
\end{align}
Since $\hat S=F_+\cup F_-$ is obtained from feasible solutions $F_+$ and $F_-$ to $\text{\sc 2DKP-Exact}(\{u_k,\hat d_k/L\}_{k\in\cN_+}, \xi_+/L,\zeta_+/L)$
 and $\text{\sc 2DKP-Exact}(\{u_k,-\hat d_k/L\}_{k\in \cN_-}, \xi_-/L,\zeta_-/L)$, respectively, and  $\xi_+ , \xi_-,\zeta_+, \zeta_-$ satisfy the condition in Step~\ref{cond1}, it follows from \raf{eq:ee1}-\raf{eq:ee3} that
\begin{align*}
\left( \sum_{k \in \hat S} d_k^{\rm R} \right)^2 +  \left(\sum_{k \in \hat S} d_k^{\rm I} \right)^2 &\le \left( \sum_{k \in \hat S} \hat d_k^{\rm R}\right)^2 +  \left(\sum_{k \in \hat S}\hat d_k^{\rm I} \right)^2+2nL\sum_{k \in \hat S_-} |\hat d_k^{\rm R}|+2n^2L^2\nonumber\\
&=(\xi_+ - \xi_-)^2 + (\zeta_+ + \zeta_-)^2 + 2nL\xi_-+2n^2L^2\nonumber\\
&\le \left((1+2\epsilon)^2C^2 +2n\frac{\epsilon}{n(P(n)+1)} C^2 + 2n^2\frac{\epsilon^2}{n^2(P(n)+1)^2}\right)C^2\\
&\le \left((1+2\epsilon)^2 +\epsilon + \frac{\epsilon^2}{2}\right)C^2\le (1+3\epsilon)^2C^2.
\end{align*}
\end{proof}

\iffalse
\begin{corollary}
For any $(\alpha, \beta)$-approximation algorithm of \textsc{CKP$[0,\pi-\delta]$} using truncated demands $\hat d_k$, we have $(\alpha, \beta (1+\epsilon))$-approximation for original demands $d_k$.
\label{cor} 
\end{corollary}
This follows immediately from Lemma~\ref{lem-trunc}. The approximation ratio $\alpha$ remains the same since any optimal $S^*$ is also feasible in the new instance within a violation of $(1+\epsilon)$.
\fi


==> frame.tex <==
%\vspace{-10pt}
\section{A Framework for Truthful-in-expectation Mechanisms}
\label{sec:frame}

In this section, we present a general framework for truthful-in-expectation mechanisms, such that our results can be applicable to a wider class of {\it packing} problems that are characterized by the existence of an approximation algorithm that rounds an LP after enumerating over a small set of partial solutions. To point out this generality we will keep our presentation as general as possible and only specialize it to problems ({\textsc{Multi-$m$DKP}) and (\textsc{multiCKP}) towards the end of this section.  


The basic idea, generalizing the one in \cite{B08}, is to approximate the feasible region $\cX^\cN$, by the integral points in a number of convex polytopes $\cQ_1,...,\cQ_r \subseteq {\cal X}$, and to show further that each $\cQ_i^{\cN} \triangleq \{ x \in {\cal Q}_i \mid x_k \in \{ 0, 1\} \mbox{\ for all\ }k \in {\cal \cN}\}$ can be written as the convex hull of the union of a polynomial number of other polytopes for which the integrality gap  can be  bounded, with a {\it polynomial-time algorithm verifying it}. Having done this, we can then apply the technique of \cite{LS05} to derive a truthful-in-expectation mechanism.  

We first recall a few definitions. We refer the reader to \cite{GLS88,S86} for more details of the theory and terminology of polyhedra and linear programming. 

%\vspace{-5pt}
\subsection{Lavi-Swamy Approach}

We briefly outline the Lavi-Swamy approach \cite{LS05}.
 
\begin{definition}\label{d1}
Let $\cQ$ be a convex polytope. Following the notations in \cite{LS05}, an algorithm is called an $\alpha$-LP-based approximation algorithm for $\cQ^{\cN}$, if for any $u\in\RR^n_+$ of polynomial support (that is, the number of non-zeros in the vector describing the objective function is polynomial in some input parameter), it returns in polynomial time an $\hat{x} \in {\cal Q}^\cN$, such that $u^T \hat{x} \ge \alpha \cdot \max_{x \in {\cal Q}} u^T x$.
\end{definition}
We emphasize that the difference between this notion and a general $\alpha$-approximation algorithm is that the latter only guarantees an $\hat{x} \in {\cal Q}^\cN$, such that $u^T \hat{x} \ge \alpha \cdot \max_{x \in {\cal Q}^\cN} u^T x$.


Lavi and Swamy \cite{LS05} proved that any $\alpha$-LP-based approximation algorithm can be combined with the VCG-mechanism to yield an $\alpha$-socially efficient truthful-in-expectation mechanism. More precisely, their result is the following. 

\begin{theorem}[\cite{LS05}]\label{t-LS}
Let $\cQ$ be a convex polytope satisfying the packing property and admitting and $\alpha$-LP-based approximation algorithm for $\cQ^{\cN}$. Then one can construct a randomized $\alpha$-socially efficient mechanism on the set of outcomes $\cQ^{\cN}$, that is truthful-in-expectation. If every basic feasible solution (BFS) of $\cQ$ has polynomial support (that is, the number of non-zeros in a BFS is polynomial in some input parameter), and one can optimize a linear function of polynomial support over $\cQ$ in polynomial time, then the mechanism is also computationally efficient.
\end{theorem}

We outline briefly the idea of the Lavi-Swamy approach. First, the VCG-mechanism is applied assuming that the space of solutions is $\cQ$ rather than $\cQ^\cN$ (that is, allowing {\it fractional allocations}; this amounts to solving a number of linear programming relaxations). The mechanism returns an optimal fractional allocation $\hat x\in\cQ$, and the corresponding VCG-payments $p_1,\ldots,p_n$. Using the $\alpha$-LP-based approximation algorithm for $\cQ^\cN$, one can obtain in polynomial-time a decomposition of $\alpha\cdot\hat x$ into a convex combination of a polynomial number of integral points from $\cQ^\cN$, i.e., write $\alpha\cdot\hat x=\sum_{\ell}\lambda_\ell x^{\ell}$, where for all $\ell$, $x^{\ell}\in\cQ^\cN$, $\lambda_\ell\ge 0$, and $\sum_{\ell}\lambda_\ell=1$. Finally, with probability $\lambda_\ell$, we return the allocation $x^\ell$ and the payments $\frac{v_k(x^\ell)}{v_k(\hat x)}p_k$, for $k=1,\ldots,n$.

%\vspace{-5pt}
\subsection{Extension to Problems with Enumerative LP-based Approximation Algorithms}\label{sec:extension}

We define some notations. Let $\cQ\subseteq[0,1]^n$ be a convex polytope. Let $\cG$ be a set of pairs $g\triangleq(g_0,g_1)$, where $g_0,g_1\subseteq\cN$ and $g_0\cap g_1=\varnothing$. For $g\in\cG$, define the convex set 
$${\cal Q}_g = \{x \in {\cal Q} \mid x_k = 0 \mbox{\ for all\ } k \in g_0 \mbox{\ and\ } x_k = 1 \mbox{\ for all\ } k \in g_1 \}.
$$ The set $\cG$ is said to be {\it complete} w.r.t. $\cQ^\cN$, if for any $x\in \cQ^\cN$ we have $x\in \cQ^\cN_g$ for some $g\in\cG$.

\begin{definition}\label{d3}
An algorithm is called an $\alpha$-enumerative LP-based approximation algorithm for $\cQ^{\cN}$, if there exists a complete set $\cG$ of size $\poly(n)$, that, for any $g\in\cG$, there is an $\alpha$-LP-based approximation algorithm for each $\cQ^\cN_g$.
\end{definition}

\begin{definition}\label{d4}
Consider a family of sets ${\cal X}_1,..., {\cal X}_r \subseteq {\cal X}$. For $\gamma\in(0,1]$, $\{{\cal X}_1,..., {\cal X}_r\}$ is called a $\gamma$-approximation to ${\cal X}$ if for all $u\in\RR^n_+$, $\displaystyle \max_{x\in \bigcup_i {\cal X}_i} u^Tx \ge \gamma\cdot\max_{x\in {\cal X}}u^T x$.
\end{definition}

\begin{definition}\label{d2}
A convex set $\cX \subseteq\RR^n_+$ satisfies the packing property if for all $x\in \cX$ and $\bzero\le y\le x$, $y\in \cX$. 
\end{definition}

It is not difficult to see that for a packing polytope $\cQ\subseteq [0,1]^n$ and a pair of sets $g=(g_0,g_1)$, $\cQ_g$ satisfies the packing property. 
\iffalse
Indeed, $\cQ$ can be written as $\cQ=\{x\in\RR^n_+ \mid Ax\le b\}$, for some real matrix $A$. Then by definition  
$$
\cQ_g=\{x\in\RR^n_+ \mid Ax\le b,~x_i=0~\forall i\in g_0\text{ and } x_i=1~\forall i\in g_1\}=\{x\in\RR^n_+ \mid A^gx\le b^g\},
$$  
where $A^g$ is the matrix obtained from $A$ by replacing each column $A_j$ with index $j\in g_0\cup g_1$ by the all-zero column, and $b^g=b-\sum_{j\in g_1}A_j$. For a vector $x\in\RR^n$ define the vector $x'$ by
$$
x'_k\triangleq\left\{\begin{array}{ll}
0&\text{if $k\in g_0$,}\\
1&\text{if $k\in g_1$,}\\
x_k& \text{otherwise.}
\end{array}\right.
$$
Suppose now that $x\in \cQ_g$ and $\bzero\le y\le x$. Then $A^g x\le b^g$ which implies that $Ax'\le b$. Since $\bzero\le y'\le x'$, we obtain by the packing property of $\cQ$ that $Ay'\leq b$, implying $A^g y\le b^g$. 
\fi

Consider a number of convex polytopes $\cQ_i\subseteq \RR^n$, for $i=1,..., r$. The convex hull of the union is given by
\begin{eqnarray}\label{chu-g}
\mbox{CvxHull}(\bigcup_{i=1}^r \cQ_i)=\{x\in\RR^n \mid x=\sum_{i=1}^rx^i,~\sum_{i=1}^r\lambda_i=1,\nonumber\\
~\lambda\ge 0,~ \forall i: x^i\in \lambda_i \cdot \cQ_i\}.
\end{eqnarray}

For instance, if $\cQ_i\triangleq\{x\in\RR^n|~A^ix\le b^i, ~x\ge 0\}$, where $A^i\in\RR^{m_g\times n}_+$ and $b^i\in\RR_+^{m_g}$, for $i=1,..., r$, then
\begin{eqnarray*}\label{chu}
\mbox{CvxHull}(\bigcup_{i=1}^r \cQ_i)=\{x\in\RR^n_+|~x=\sum_{i=1}^rx^i,~\sum_{i=1}^r\lambda_i=1,\\~\lambda\ge 0,~ \forall i: A^ix^i\le \lambda_ib^i, ~ x^i\ge 0\}.
\end{eqnarray*}
It is well-known \cite{B98} and also easy to see that each {\it extreme point (basic feasible solution (BFS) in case of convex polytope)} of \raf{chu-g} corresponds to an extreme point of some $\cQ_i$, that is, it has $\lambda_i=1$ for some $i$.

\medskip

We will need that the convex hull of the union of a number packing polytopes is also a packing polytope.  
\begin{lemma}\label{pack}
Let $\cQ_i\triangleq\{x\in\RR^n_+|~A^ix\le b^i\}$, where $A^i$ are matrices such that $\cQ_i$ is packing for $i=1,...,r$ (e.g., $A^i$ can be non-negative). Then $\cQ\triangleq\mbox{CvxHull}(\bigcup_{i=1}^r \cQ_i)$ satisfies the packing property. 
\end{lemma}
\iffalse
\begin{proof}
%It is enough to show the claim for $G=2$.
Write $\cQ$ as in \raf{chu}. Suppose $x\in \cQ$ and $\bzero\le y\le x$. Then there exist $x^1,..., x^r\in\RR^n_+$ and $\lambda_1,...,\lambda_r\ge 0$, s.t. $\sum_{i=1}^{r}\lambda_i=1$, $x=\sum_{i=1}^rx^i$, $A^ix^i\le\lambda_ib^i$, for $i=1,..., r$. For $k=1,..., n$, set iteratively, $$y_k^i\triangleq \min\left\{\max\{0,y_k-\sum_{i'=1}^{i-1}y_j^{i'}\},x_k^i\right\},$$
for $i=1,...,r-1$, and set $y^r\triangleq y-\sum_{i=1}^{r-1}y^i$. Then by definition, $y=\sum_{i=1}^r y^i$ and $\bzero\le y^i\le x^i$, for $i=1,..., r$. The latter condition  implies by the packing property of $\cQ_i$ that $A^iy^i\le A^ix^i\le \lambda_ib^i$, that is, $y\in \cQ$.   
\end{proof}
\fi
The following result generalizes the ideas from \cite{B08} and \cite{P10}.

\begin{proposition}\label{t-convert}
Let $\cX\subseteq [0,1]^n$ be a compact convex set, and  $\cQ_1,...,\cQ_r\subseteq \cX$ be a set of convex polytopes, such that $\{\cQ_1^\cN,...,\cQ_r^\cN\}$ $\gamma$-approximates $\cX^\cN$, where $\cQ_i$ has $f_i$ facets. Suppose that, for each $i=1,...,r$, there exists an $\alpha$-enumerative LP-based approximation algorithm for $\cQ^{\cN}_i$. Then there exists a convex polytope $\widehat \cQ\subseteq \RR^n$ such that 
\begin{itemize}
\item [(i)] $\widehat \cQ\subseteq \cX$ and $\widehat \cQ$ has $\poly(n)\cdot\sum_{i=1}^r f_i$ facets; if for all $i=1,...,r$, $\cQ_i$ is packing, then $\widehat \cQ$ is packing;  
\item[(ii)] there is an $\alpha$-LP-based approximation algorithm $\cB$ for $\widehat \cQ^\cN$; moreover,
for any $u\in\RR^n_+$, $\cB$ returns, in polynomial time, an $\tilde x\in \cX^\cN$, such that $u^T\tilde x\ge \alpha \gamma\cdot \max_{x\in \cX^\cN} u^Tx$. 
\end{itemize}
\end{proposition}
\begin{proof}
By assumption, for each $i=1,...,r$ there is a complete set $\cG_i$ of size $\poly(n)$, such that, for any $g\in\cG_i$, the polytope $(\cQ_i)_g$ has an $\alpha$-LP-based approximation algorithm $\cA_{i,g}$. Let $\widehat \cQ\triangleq\mbox{CvxHull}(\bigcup_{i,g} (\cQ_i)_g)$. Then $\widehat Q$ satisfies the first part in $(i)$; the second part follows from Lemma \ref{pack}.
Since $\cG_i$ is complete, $\cQ_i^\cN\subseteq\bigcup_{g\in \cG_i}(\cQ_i)_g^\cN\subseteq\widehat \cQ^\cN$, and it follows by the $\gamma$-approximation assumption that, for all $u\in\RR^n_+$,
\begin{equation*}\label{ce1}
\max_{x\in\widehat \cQ^\cN}u^Tx\ge\max_{i=1,...,r}\max_{x\in\cQ_i^\cN}u^Tx\ge \gamma\cdot\max_{x\in \cX^\cN}u^Tx.
\end{equation*}
To show (ii), we give the algorithm $\cB$. Consider any $u\in\RR^n_+$. Let $\hat x$ be an optimal BFS of $\widehat \cQ$ w.r.t. objective $u$. Then $\hat x$ is a BFS of $(\cQ_i)_g$ for some $i=1,...,r$ and $g\in\cG_i$. We apply $\cA_{i,g}$ on $\hat x$ to return an $\tilde x\in  (\cQ_i)_g^\cN\subseteq \widehat \cQ^\cN\subseteq \cX^\cN$ such that $u^T\tilde x\ge \alpha\cdot u^T\hat x  \ge \alpha\cdot \max_{x\in\widehat \cQ^\cN}u^Tx \ge  \alpha\gamma\cdot \max_{x\in \cX^\cN} u^Tx$.
\end{proof}

%\begin{corollary}\label{t-MIP}
%Let $Q\subseteq [0,1]^n$ be a compact convex set, and  $Q_1,\ldots,Q_r\subseteq Q$ be a set of convex polytopes such that  the set $\{Q_1^\cN,\ldots,Q_r^\cN\}$ $\gamma$-approximates $Q^\cN$. Suppose that, for each $i\in[r]$ and $x\in Q$, there exists an $(\alpha,\beta)$-enumerative LP-based approximation algorithm for $Q^{\cN}_i$. Then, there is an $(\alpha\gamma,\beta)$-approximation algorithm for solving the problem $\max_{x\in Q^\cN}u^Tx$. 
%\end{corollary}

We now combine the construction in Proposition \ref{t-convert} with the results in \cite{LS05} to obtain a truthful-in-expectation mechanism for problems that admit an enumerative LP-based approximation algorithm. 

%We shall extend Theorem~\ref{t-LS} as follows.

\begin{theorem}\label{t-TIE}
Let ${\cal X} \subseteq [0,1]^n$ be a compact convex set, and  $\cQ_1,\ldots,\cQ_r\subseteq {\cal X}$ be a set of convex polytopes, such that the set $\{\cQ_1^\cN,...,\cQ_r^\cN\}$ $\gamma$-approximates $\cX^\cN$ and the dimension of each $\cQ_i$ is part of the input. Suppose that, for each $i=1,\ldots,r$, there exists an $\alpha$-enumerative LP-based approximation algorithm for $\cQ_i^\cN$. Let $\widehat \cQ$ be the polytope constructed in Proposition \ref{t-convert}. Then one can construct a randomized $\alpha\gamma$-socially efficient mechanism on the set of outcomes $\cX^{\cN}$, that is truthful in expectation. If one can optimize a linear function of polynomial support over $\widehat{\cQ}$ in polynomial time, then the mechanism is also computationally efficient. 
\end{theorem}


\begin{proof}
By Proposition \ref{t-convert}-(ii), $\widehat{\cQ}^\cN$ has an $\alpha$-LP based-approximation algorithm $\cA$ whose output is always an element in $\cX^\cN$.  
Theorem \ref{t-LS} implies that there exists a mechanism which is truthful-in-expectation, individually rational, with no positive transfer, and which is $\alpha$-socially efficient on the set of outcomes $\widehat \cQ^\cN$.
Thus, the expected social welfare output by the mechanism is at least $\alpha\cdot \max_{x\in\widehat \cQ^\cN}v(x) \ge  \alpha\gamma\cdot \max_{x\in \cX^\cN} v(x)$.  
\end{proof}

\iffalse
{\bf Remark:}
Algorithmically, Theorem \ref{t-TIE} can be obtained by directly enumerating over all possible $g\in \bigcup_{i\in [r]} \cG_i$ and modifying the LS-technique to work over the space of enumerated solutions. However the construction of the polytope $\widehat \cQ$ is neater in the sense that, it allows us to use black-box reductions without the need to look inside them.     
\fi

We shall give two applications of Theorem \ref{t-TIE}. In the first one, we consider the  
multiple choice-multi dimensional knapsack problem, for which there is a PTAS \cite{FC84alg}, and bi-criteria truthful FPTAS \cite{KTV13}. Here, we point out that a truthful-in-expectation PTAS follows from Theorem \ref{t-TIE}. As a special case of this, we obtain a truthful-in-expectation PTAS  for multi-unit combinatorial auctions with a {\it constant} number of distinct goods, for which a bi-criteria FPTAs was given recently in \cite{KTV13}. Finally, we extend this result to {\sc CKP}$[0,\frac{\pi}{2}]$. 
    
%\vspace{-5pt}
\subsection{A Truthful-in-expectation PTAS for \textsc{Multi-$m$DKP}}
%Multiple-choice Multidimensional Knapsack Problem}
\label{sec:Tm-mC-KS}
The single-minded $m$DKP problem was shown in \cite{FC84alg} to have a $(1-\epsilon)$-enumerative-LP-based approximation algorithm. We show first that this can be extended to the multi-minded variant of the problem.

Consider the polytope $\cP$ defined by the relaxation \raf{mCmD-1}-\raf{mCmD-3}. 
%Assume w.l.o.g. that $n\ge h\triangleq m^2/\epsilon$.
Define $h\triangleq \min\{n,m^2/\epsilon\}$.  
Let $\cO\subseteq\cN\times\cD$ be an optimal integral solution, that is, with the additional constraints $x_{k,d}\in\{0,1\}^{\cN\times\cD}$, and let $\OPT$ be the value of such a solution.
Let $\bar g=(\bar g(1),..., \bar g(m))$ be an $m$-vector of $h$-tuples of pairs (that is, $m$ vectors each having $h$ components, each of which is a pair): $\bar g(i) =((k(i,j),d(i,j)) \mid j=1,...,h)$, $i\in[m]$; here $d(i,j)\in\cD$ stands for the $j$-th largest demand in $\cO$ w.r.t the $i$-th constraint (that is, if we order the demands $d\in\RR^m$ such that $x_{k,d}=1$ in $\cO$, according to the $i$-th component $d^i$ in $d$) and $k(i,j)\in\cN$ stands for the index of the user allocated such demand. For every such $\bar g$ we can associate a pair of sets $g=(g_0,g_1)$, such that $g_0,g_1\subseteq\cN\times\cD$ are defined as follows: 

{\small
\begin{eqnarray}\label{Pg}
g_1&=&\{(k(i,j),d(i,j))\mid i=1,...,m,~j=1,...,h\}\nonumber\\
g_0&=&\{(k(i,j),d)\mid i=1,...,m,~j=1,...,h,~d\in\cD,~d\ne d(i,j)\}\cup\nonumber\\
&&~~\{(k,d)\in \cN\times\cD\mid (k,d)\not\in g_1\text{ and $\exists i:$ }  d^i > \min_{(k',d')\in g_1}d^i(k',d')\}.\nonumber
\end{eqnarray}}
Let $\cG\triangleq\{g~|~\cP_g\neq\emptyset\}$. Using the notation of Section \ref{sec:frame}, we note that the set $\cG$ is complete w.r.t. $\cP^\cN$.  
\iffalse
We will make use of the following lemma in Section \ref{sec:Tm-mC-KS}.

\begin{lemma}[\cite{SR10}]\label{lll1}
Let $x$ be an extreme point in $\cP$. Then $x$ has at most $2m$ non-integral components. 
\end{lemma}
\begin{proof}
Let $h$ be the number of users $k$ such that $\sum_{d\in\cD}x_{k,d}=1$.  
By the properties of a BFS (see, e.g., \cite{GLS88,S86}), the number of strictly positive components in $x$ is at most $m+h$. Furthermore, constraints \raf{mCmD-2} impose that for each $k\in\cN$, among those $h$ users, there is a $d\in\cD$ such that $x_{k,d}>0$. The remaining $m$ positive variables can belong to at most $m$ of the constraints \raf{mCmD-2}, implying that at least $\max\{h-m,0\}$ variables are set to $1$. It follows that the total number variables taking non-integral values is at most $m+h-\max\{h-m,0\}\le 2m$.  
\end{proof}
\fi


The following lemma, which is based on a generalization of the rounding procedure in \cite{P10}, shows the existence of an $(1-\epsilon)$-enumerative LP-based approximation algorithm for $\cP^\cN$.
%\vspace*{-5pt}
\begin{lemma}\label{lll2}
Let $\hat x$ be a point in $\cP_g$ of polynomial support, for some $g\in\cG$. Then we can find in polynomial time an integral solution $x^*$ to \raf{mCmD-1}-\raf{mCmD-3} s.t. $\sum_{k\in\cN}\sum_{d\in\cD}v_k (d)x^*_{k,d}\ge (1-\epsilon)\sum_{k\in\cN}\sum_{d\in\cD}v_k (d)\hat x_{k,d}$.
\end{lemma}
\iffalse
\begin{proof}
W.l.o.g. we may assume that $\hat x$ is a BFS of $\cP_g$. We may also assume that $n\ge m/\epsilon^2$, for otherwise $\cP_g$ consists of single integral point.
By (the proof of) Lemma \ref{lll1}, there exist at most $m$ users $k$ for which $\hat x_{k,d}\in(0,1)$ for some $d\in\cD$. For each such $k$, we set $x^*_{k,d}$ to $1$ with probability $\hat x_{k,d}$ (for instance, standardly, by picking a $\delta\in[0,1]$ at random and setting, for each $k\in\cN$, $x^*_{k,d}=1$ according to the following procedure: order the set of non-zero variables $\hat x_{k,d}$ arbitrarily, say, in the order, $\hat x_{k,d_k(1)},\hat x_{k,d_k(2)}, \ldots$; then set $ x^*_{k,d_k(i)}=1$, where $i$ satisfies $\sum_{j=1}^{i-1}\hat x_{k,d_k(i)}<\delta\leq \sum_{j=1}^{i}\hat x_{k,d_k(i)}$; this rounding procedure can be easily derandomized since the number of different choices of $\delta $ by Lemma \ref{lll1} is at most $2m$). This way, we obtain an integral solution $x^*_{k,d}$ with expected utility $\sum_{k\in\cN}\sum_{d\in\cD}v_k (d)\hat x_{k,d}$, but in which some of the constraints in \raf{mCmD-1} are possibly violated. To remove the violations, we consider these constraints in some order, and remove some of the demands, until all the constraints are satisfied. More precisely, suppose that the demands assigned to the $n$ users by the solution $x^*$ are $d_1,..., d_n$. When we consider the $i$-th constraint in  \raf{mCmD-1}, we order the users in non-decreasing order by the value of $v_k(d_k)$ and drop demands (that is, set $x_{k,d_k}^*=0$) in that order, until the constraint is satisfied. Note that we do not need to drop more than $m$ demands in each constraint. The reasons are (i) $\hat x$ was feasible and, by Lemma \ref{lll1}, the number of demands added after rounding the fractional components is at most $m$; and (ii) let $g=(g_0,g_1)$ be associated with the guess $\bar g\triangleq(\bar g(1),...,\bar g(m))$, where $\bar g(i) =((d(i,j),k(i,j)) \mid j=1,...,h)$, then all the added demands $d$ have $d^i\le d^i(i,j)$ for all $j=1,\ldots,h$ (by the definition of $\cP_g$), and hence dropping at most $m$ demands from the set $\{d(i,j) \mid j=1,...,h\}$ would be enough to restore feasibility in the $i$-th constraint. It follows that the total number of dropped demands is at most $m^2$ and their total value is  bounded by 
$\frac{m^2}{h}\sum_{(k,d)\in g_1}v_k(d)\le\epsilon\sum_{k\in\cN}\sum_{d\in\cD}v_k (d)\hat x_{k,d}$. 
\end{proof}
\fi
\begin{corollary}\label{Multi-$m$DKP}
There is a PTAS for {\sc Multi-$m$DKP}.
\end{corollary}
%\vspace*{-5pt}
The following theorem follows from the observation at the end of Section~\ref{MCMDKP-sec}, in conjunction with Theorem~\ref{t-TIE} and Lemma \ref{lll2}. 
\begin{theorem}\label{t-TIE-mCmD-KS}
Assume that $|\cD|=\poly(n)$, or each $v_k(\cdot)$ is a multi-minded valuation defined by \raf{mm-val}. Then, for any $\epsilon>0$ there is a computationally efficient randomized, individually rational, $(1-\epsilon,1)$-socially efficient mechanism, for the multiple choice multi-dimensional knapsack problem, that is truthful-in-expectation and has no positive transfer.
\end{theorem}
\begin{proof}
We apply Theorem~\ref{t-TIE} with $\cX=\cP$. Let $\widehat \cQ\triangleq \mbox{CvxHull}(\bigcup_{g\in\cG} \cP_g)$.
We need to show that: (i) we can find $x^*$ maximizing $\sum_{k\in\cN}\sum_{d\in\cD}v_k(d)x_{x,d}$ over all $x\in\widehat\cQ$, in polynomial time, and (ii) we can optimize a linear function of polynomial support over $\widehat \cQ$, in polynomial time. Claim (ii) follows easily form the fact that the objective function has a polynomial support.   
If $|\cD|=\poly(n)$ then the first claim is also immediate, since we have an explicit construction. Now, consider the case when each $v_k(\cdot)$ is a multi-minded valuation function. Let $\widehat{\cD}$ be the set of {\it component-wise minimal} vectors $d\in\cD$ such that $d\succeq d'$ for all $d'\in S$ and some $S\subseteq\bigcup_{k\in\cN} D_k$. Note that $|\widehat\cD|\le \left(\sum_{k}|D_k|\right)^m$ since each element in $\widehat\cD$ is determined by $m$ hyperplanes from the set $\{\{x\in\RR^m:~x_i\ge d_i\}\mid d\in\bigcup_{k\in\cN} D_k\}$.  
To see (i), we argue that there is an optimal solution $x\in\widehat\cQ$ s.t. that, for $k\in\cN$, $x_{k,d}>0$ implies that $d\in \widehat\cD$. Given an optimal BFS $x^*\in\widehat\cQ$ which violates this property, we modify it to another optimal solution satisfying the property as follows. Suppose $x^*\in\cP_g$ for some $g=(g_0,g_1)\in\cG$, $x^*_{k,d}>0$, and $d\not \in \widehat\cD$. Let $d'\in D_k$ be such that $d'\preceq d$ and $v_k(d')=v_k(d)$; we consider two cases:

\noindent {\it Case 1.} $(k,d)\not\in g_1$: Note that $(k,d')\not\in g_0\cup g_1$ (since $x^*_{k,d}>0$). Set $x^*_{k,d}\leftarrow 0$ and $x^*_{k,d'}\leftarrow x^*_{k,d'}+x^*_{k,d}$. Then, it follows from the packing property of $\cP_g$ that the new $x^*$ is also in $\cP_g$.

\noindent {\it Case 2.} $(k,d)\in g_1$: for every pair $(\bar k,\bar d)\not\in g_0\cup g_1$ s.t. $d'\preceq \bar d\preceq d$, we first ensure, by applying Case 1, that $x^*_{\bar k,\bar d}>0$ only for some $\bar d\in D_{\bar k}$ such that $\bar d'\preceq \bar d$ and $v_{\bar k}(\bar d')=v_{\bar k}(\bar d)$.
Next, we let $S$ be the set of all such $\bar d'$s, and $\hat d$ be the component-wise minimal vector such that $\hat d\succeq \bar d'$ for all $\bar d'\in S$ and $d'\succeq d$. Now, we have that the new $x^*$ is a feasible point in $P_{g'}$ for some $g'\in\cG$ which is obtained from $g$ by setting $g_0\leftarrow g_0 \cup\{(k,d)\}\setminus\{(k,\hat d)\}$ and $g_1\leftarrow g_1 \cup\{(k,\hat d)\}\setminus\{(k,d)\}$.

It easy to see that in both cases the resulting modified solution $x^*$ retains the same objective value.  Thus, we may as well assume for  the purpose of computing $x^*$ that $\widehat\cQ$ is constructed under the assumption that $\cD=\widehat\cD$.  
\end{proof}



